Spectral Modelling of H.E.S.S.-detected Pulsar Wind Nebulae

In the last decade, ground-based Imaging Atmospheric Cherenkov Telescopes have discovered about 175 very-high-energy (VHE; $E >$ 100 GeV) gamma-ray sources, with more to follow with the development of H.E.S.S. II and CTA. Nearly 40 of these are confirmed pulsar wind nebulae (PWNe). We present results from a leptonic emission code that models the spectral energy density of a PWN by solving a Fokker-Planck-type transport equation and calculating inverse Compton and synchrotron emissivities. Although models such as these have been developed before, most of them model the geometry of a PWN as that of a single sphere. We have created a time-dependent, multi-zone model to investigate changes in the particle spectrum as the particles traverse through the PWN, by considering a time and spatially-dependent magnetic field, spatially-dependent bulk particle motion causing convection, diffusion, and energy losses (SR, IC and adiabatic). Our code predicts the radiation spectrum at different positions in the nebula, yielding novel results, e.g., the surface brightness versus the radius and the PWN size as function of energy. We calibrated our new model against more basic models using the observed spectrum of PWN G0.9+0.1, incorporating data from H.E.S.S. as well as radio and X-ray experiments. We fit our predicted radiation spectra to data from G21.5$-$0.9, G54.1+0.3, and HESS J1356$-$645 and found that our model yields reasonable results for young PWNe. We next performed a parameter study which gave significant insight into the behaviour of the PWN for different scenarios. Our model is now ready to be applied to a population of PWNe to probe possible trends such as the surface brightness as a function of spin-down of the pulsar.

==> Space.tex <==
% Chapter 3
\clearpage
\chapter{Spatial dependent Results from PWN Model} % Write in your own chapter title
\label{ch:Space}
\lhead{Chapter \ref{ch:Space}. \sc{Spatial dependent Results from PWN Model}} % Write in your own chapter title to set the page header
The code created to model the PWNe is a spacial dependent model which means that it is possible to show results about the morphology of the PWN. This chapter is therefore dedicated to show the changes in the PWN's morphology when certain parameters are changed. 

\section{}\label{sec:}

\begin{figure}[h]
\begin{minipage}[b]{6in}
\includegraphics[width=6in]{Kappa_123.pdf}
\caption{\label{fig:sp_kappa}Change in $\kappa$}
\end{minipage} 
\end{figure}

In Figure \ref{fig:sp_kappa} the value of kappa was changed. The solid line is for normal Bohm diffusion ($\kappa$), the dashed line is for $5\kappa$ and the dashed dotted line is for $\kappa/5$. 
\clearpage

\begin{figure}[h]
\begin{minipage}[b]{6in}
\includegraphics[width=6in]{G09+07_123_V.pdf}
\caption{\label{fig:sp_V1}Effects of $V_0$}
\end{minipage} 
\end{figure}
In Figure \ref{fig:sp_V1} the solid line shows for an unchanged $V_0$ and the dashed line shows for $V_0 = 0$.


\clearpage

\begin{figure}[h]
\begin{minipage}[b]{6in}
\includegraphics[width=6in]{G09+07_456_V.pdf}
\caption{\label{fig:sp_V2}}
\end{minipage} 
\end{figure}

In Figure \ref{fig:sp_V2} the solid line shows for an unchanged $V_0$, the dashed line shows for $10 V_0$ and the dashed dotted line is for $V_0/10$.




\clearpage

\begin{figure}[h]
\begin{minipage}[b]{6in}
\includegraphics[width=6in]{SizevEnergy_K.pdf}
\caption{\label{fig:SvE_k}Change in kappa}
\end{minipage} 
\end{figure}


\clearpage

\begin{figure}[h]
\begin{minipage}[b]{6in}
\includegraphics[width=6in]{SizevEnergy_V.pdf}
\caption{\label{fig:SvE_V}Change in V}
\end{minipage} 
\end{figure}











